Reinforcement Learning Meets Large Language Models: A Survey of Advancements and Applications Across the LLM Lifecycle

In recent years, training methods centered on Reinforcement Learning (RL) have markedly enhanced the reasoning and alignment performance of Large Language Models (LLMs), particularly in understanding human intents, following user instructions, and bolstering inferential strength. Although existing surveys offer overviews of RL augmented LLMs, their scope is often limited, failing to provide a comprehensive summary of how RL operates across the full lifecycle of LLMs. We systematically review the theoretical and practical advancements whereby RL empowers LLMs, especially Reinforcement Learning with Verifiable Rewards (RLVR). First, we briefly introduce the basic theory of RL. Second, we thoroughly detail application strategies for RL across various phases of the LLM lifecycle, including pre-training, alignment fine-tuning, and reinforced reasoning. In particular, we emphasize that RL methods in the reinforced reasoning phase serve as a pivotal driving force for advancing model reasoning to its limits. Next, we collate existing datasets and evaluation benchmarks currently used for RL fine-tuning, spanning human-annotated datasets, AI-assisted preference data, and program-verification-style corpora. Subsequently, we review the mainstream open-source tools and training frameworks available, providing clear practical references for subsequent research. Finally, we analyse the future challenges and trends in the field of RL-enhanced LLMs. This survey aims to present researchers and practitioners with the latest developments and frontier trends at the intersection of RL and LLMs, with the goal of fostering the evolution of LLMs that are more intelligent, generalizable, and secure.

==> overview.tex <==
\definecolor{mc1}{RGB}{109,173,209}
\definecolor{mc2}{RGB}{182,215,232}
\definecolor{mc3}{RGB}{233,241,244}
\definecolor{mc4}{RGB}{233,241,244}
\definecolor{mcleaf}{RGB}{251,227,213}
\definecolor{data}{HTML}{F8CECC}
\definecolor{learn}{HTML}{DAE8FC}
\definecolor{constraint}{HTML}{D5E8D4}
\definecolor{model}{HTML}{FFF2CC}
\definecolor{dpo}{HTML}{F9F7ED}

\tikzstyle{my-box}=[
    rectangle,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=6em,
    inner sep=3pt,
    align=center,
    fill opacity=.3,
    thick,
]
\tikzstyle{leaf}=[
    my-box, 
    fill=gray!3, % 柔和青色
    text=black, 
    align=left,
    text width=53em,
    font=\normalsize,
    inner xsep=3pt,
    inner ysep=4pt,
]
\begin{figure*}[!t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\normalsize,
                rectangle,
                draw=gray,
                rounded corners,
                align=left,
                text centered,
                minimum width=5em,
                edge+={gray!60, thick},
                s sep=4pt,
                inner xsep=3pt,
                inner ysep=3pt,
                thick,
                fit=band,
            },
            where level=0{
                folder,
                grow'=0,
                fill=dpo,
                font=\large,
                child anchor=west,
                parent anchor=south west,
                anchor=west,
                calign=first,
                yshift=120pt,
            }{},
            where level=1{
                text width=14em,
            }{},
            where level=2{text width=10em}{},
            where level=3{text width=9em}{},
            [
                {\quad\quad\qquad\qquad\quad{\textbf{A Taxonomy of Direct Preference Optimization (DPO)}}\qquad\qquad\qquad
                \begin{minipage}[h]{0.68\textwidth}
                    \centering
                    \includegraphics[width=\linewidth]{fig/dpo.pdf}
                \end{minipage}\qquad\qquad\qquad\qquad}
                [
                    \textbf{Data Strategy (\S \ref{sec:data})}, fill=data
                    [
                        \textbf{Quality (\S \ref{sec:quality})}, fill=data
                        [
                            \textbf{Heterogeneity}, fill=data
                            [   
                                MinMax-DPO~\cite{chidambaram2024direct}{, }
                                MallowsPO~\cite{chen2024mallowspo}{, }
                                GRPO~\cite{ramesh2024group}{, }
                                GDPO~\cite{yao2025no}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Distinguishability}, fill=data
                            [
                                ODPO~\cite{amini2024direct}{,} 
                                MPO~\cite{gou2024mixed}{,} 
                                DPO-rc~\cite{wang2024reward}{,} 
                                $\alpha$-DPO~\cite{wu2024alpha}{,}
                                GDPO~\cite{furuta2024geometric}{,} 
                                $\beta$-DPO~\cite{wu2024betadpo}{,}
                                fDPO~\cite{morimura2024filtered}{, } 
                                Curri-DPO~\cite{pattnaik2024enhancing}{,} \\
                                Ada-DPO~\cite{hong2024adaptive}{,} 
                                sDPO~\cite{kim2024sdpo}{,} 
                                Sr-DPO~\cite{yu2024direct}{,} 
                                GaPO~\cite{jieming2024gapaware}{, }
                                \citet{ma2024plugandplay} 
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Noise}, fill=data
                            [
                                rDPO~\cite{chowdhury2024provably}{,} 
                                PerpCorrect~\cite{kong2024perplexityaware}{,} 
                                ROPO~\cite{liang2024ropo}{,} 
                                SPA~\cite{kim2025spread}{,} 
                                \citet{zhang2025combating}{,} 
                                \citet{im2025understanding}{,} 
                                \citet{gao2024impact}{,} 
                                \citet{wu2024towards} 
                                , leaf
                            ]
                        ]
                    ]
                    [
                        \textbf{Feedback  (\S \ref{sec:feedback})}, fill=data
                        [
                            \textbf{Point-Wise}, fill=data
                            [                            
                                KTO~\cite{ethayarajh2024kto}{, }
                                BCO~\cite{jung2024binary}{, }
                                Cal-DPO~\cite{globerson2024cal}{, }
                                DRO~\cite{wu2024towards}{, }
                                AOT~\cite{melnyk2024distributional}{, }
                                ULMA~\cite{cai2023ulma}{, }
                                NCA~\cite{chen2024noise}{, } 
                                GPO~\cite{zhang2024general}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Pair-Wise}, fill=data
                            [
                                DPO~\cite{rafailov2024direct}{,}
                                IPO~\cite{azar2024general}{,}
                                DPO-RK~\cite{chen2024extending}{,} 
                                DPO-D~\cite{chen2024extending}{,}
                                BMC~\cite{jiang2024bridging}{,}
                                IOPO~\cite{zhang2024iopo}{,}
                                PMPO~\cite{abdolmaleki2024preference}{,} 
                                SAPO~\cite{yin2024self}{, }
                                D2O~\cite{duan2024negating}{, }\\
                                NPO~\cite{zhang2024negative}{, }
                                SimNPO~\cite{fan2024simplicity}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{List-Wise}, fill=data
                            [
                                Panacea~\cite{zhong2024panacea}{,}
                                LiPO~\cite{liu2402lipo}{,}
                                LIRE~\cite{zhu2024lire}{,}
                                OPO~\cite{zhao2024ordinal}{,}
                                DRPO~\cite{zhou2024optimizing}{,}
                                mDPO~\cite{wang2024mdpo}{,} 
                                RPO~\cite{yin2024relative}{,} 
                                TODO~\cite{guo2024todo}
                                , leaf
                            ]
                        ]
                    ]
                    [
                        \textbf{Granularity  (\S \ref{sec:granularity})}, fill=data
                        [
                            \textbf{Token-Level}, fill=data
                            [    
                                \citet{rafailov2024from}{, }
                                TDPO~\cite{zeng2024token}
                                TIS-DPO~\cite{liu2024tis}{, }
                                SparsePO~\cite{christopoulou2024sparsepo}{, }
                                RTO~\cite{zhong2024dpo}{, }
                                SePO~\cite{yang2024selective}{, } 
                                EPO~\cite{qi2024epo}{, }
                                D$^2$PO~\cite{shao2025earlier}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Step-Level}, fill=data
                            [
                                Step-DPO~\cite{lai2024step}{,} 
                                SCDPO~\cite{lu2024step}{,} 
                                CPO~\cite{zhang2024chain}{,} 
                                MCTS-DPO~\cite{xie2024monte}{,} 
                                TPO~\cite{liao2024tpo}{,} 
                                RDPO~\cite{just2024data}{,}  
                                DAPO~\cite{liu2024improving}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Sentence-Level}, fill=data
                            [
                                DPO~\cite{rafailov2024direct}{,} 
                                MAPO~\cite{she2024mapo}{,} 
                                EURUS~\cite{yuan2024advancing}{,} 
                                IRPO~\cite{pang2025iterative}{,} 
                                FACTALIGN~\cite{huang2024factalign}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Turn-Level}, fill=data
                            [
                                M-DPO~\cite{xiong2024building}{,} 
                                ETO~\cite{song2024trial}{,} 
                                SDPO~\cite{kong2025sdpo}{,} 
                                AgentQ~\cite{putta2024agent}{, }
                                DMPO~\cite{shi2024direct}
                                , leaf
                            ]
                        ]
                    ]
                ]
                [
                    \textbf{Learning Framework (\S \ref{sec:learning})}, fill=learn
                    [
                        \textbf{Paradigm  (\S \ref{sec:paradigm})}, fill=learn
                        [
                            \textbf{Offline}, fill=learn
                            [                            
                                DPO~\cite{rafailov2024direct}{,}
                                CPO~\cite{xu2024contrastive}{,}
                                ORPO~\cite{hong2024orpo}{,}
                                ULMA~\cite{cai2023ulma}{,}
                                PAFT~\cite{pentyala2024paft}{,} 
                                Curri-DPO~\cite{pattnaik2024enhancing}{,} 
                                sDPO~\cite{kim2024sdpo}{,} \\
                                Linear Alignment~\cite{gao2024linear}{,}
                                ICDPO~\cite{song2024icdpo}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Online}, fill=learn
                            [
                                OAIF~\cite{guo2024direct}{,}
                                OFS-DPO~\cite{qi2024online}{,}
                                \citet{yuan2024selfrewarding}{,}
                                BPO~\cite{xu2024bpo}{,}
                                RS-DPO~\cite{khaki2024rs}{,} 
                                RSO~\cite{liu2024statistical}{,} 
                                ROPO~\cite{liang2024ropo}{,}
                                \citet{shi2024crucial}{,} \\
                                OPTUNE~\cite{chen2024optune}{,}
                                Iterative RPO~\cite{pang2025iterative}{,} 
                                DPO-ST~\cite{wang2024self}{,}
                                \citet{xie2024monte}{,} 
                                APO~\cite{he2024accelerated}{,}
                                \citet{xiong2023iterative}{,}
                                COMAL~\cite{liu2024comal}{,}\\
                                \citet{xu2024things}{,}
                                SeRA~\cite{ko2024sera}{,}
                                CREAM~\cite{wang2024cream}{,}
                                D2PO~\cite{singhal2024dpo}{,}
                                DLMA~\cite{liu2024direct}{,}
                                XPO~\cite{xie2025exploratory}{,}
                                SELM~\cite{zhang2024self}{,}
                                ETO~\cite{song2024trial}{,}\\
                                VPO~\cite{cen2024value}{,}
                                \citet{xiong2024building}{,}
                                COPO~\cite{bai2025online}{,}
                                HyPO~\cite{song2024importance}{,}
                                MPO~\cite{gou2024mixed}{,}
                                AIPO~\cite{shen2024aipo}{,}
                                \citet{tang2024understanding}{,} 
                                \citet{xu2024is}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Active}, fill=learn
                            [
                                APL~\cite{muldrew2024active}{,}
                                divAPO~\cite{choi2024active}{,}
                                ADPO\cite{ji2024reinforcement}{,}
                                \citet{das2024active}
                                , leaf
                            ]
                        ]
                    ]
                    [
                        \textbf{Objective  (\S \ref{sec:objective})}, fill=learn
                        [
                            \textbf{Multi-Objective}, fill=learn
                            [
                                MODPO~\cite{zhou2024beyond}{,}
                                SPO~\cite{lou2024spo}{,}
                                MOSLIM~\cite{zhang2025moslimalign}{,}
                                HPO~\cite{badrinath2024hybrid}{,}
                                CPO~\cite{guo2024controllable}{,}
                                DRDO~\cite{nath2024simultaneous}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Self-Play}, fill=learn
                            [                            
                                SPIN~\cite{chen2024self}{,} 
                                SPPO~\cite{wu2024self} {,} 
                                SPO~\cite{swamy2024minimaximalist}{,} 
                                BoNBoN~\cite{gui2406bonbon}{,} 
                                Nash-MD~\cite{munos2023nash}{,}  
                                DNO~\cite{rosset2024direct}{,}
                                IPO-MD~\cite{calandriello2024human}{,} \\
                                SRPO~\cite{choi2024self}{,}
                                DNPO~\cite{yang2025dynamic}
                                , leaf
                            ]
                        ]
                    ]
                ]
                [
                    \textbf{Constraint Mechanism (\S \ref{sec:constraint})}, fill=constraint
                    [
                        \textbf{Reference  (\S \ref{sec:reference})}, fill=constraint
                        [
                            \textbf{Dynamic}, fill=constraint
                            [                            
                                Curri-DPO~\citep{pattnaik2024enhancing}{,} 
                                MPO~\citep{gou2024mixed}{,} 
                                M-DPO~\citep{wang2024mdpo}{,} 
                                \citet{gorbatovski2024learn}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Free}, fill=constraint
                            [
                                ORPO~\cite{hong2024orpo}{, } 
                                SimPO~\cite{Meng2024simpo}{, }
                                SimPER~\cite{xiao2025simper}{, }
                                \citet{liu2024understanding}{, }
                                \citet{xu2024contrastive}
                                , leaf
                            ]
                        ]
                    ]
                    [
                        \textbf{Divergence  (\S \ref{sec:divergence})}, fill=constraint
                        [
                            \textbf{Diversity}, fill=constraint
                            [                            
                                f-DPO~\cite{wang2023beyond}{, } \citet{slocum2025diverse}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Generalization}, fill=constraint
                            [
                                DPO-Kernels~\cite{das2025dpo}{,}
                                FlipGuard~\cite{zhu2024flipguard}{,}
                                FPO~\cite{yin2024direct}{,}
                                GPO~\cite{tang2024generalized}{,} 
                                EXO~\cite{ji2024towards}{, } 
                                SPO~\cite{sharifnassab2024soft}{, }
                                QDPO~\cite{lee2024improving}{, }
                                \citet{huang2025correcting}
                                , leaf
                            ]
                        ]
                    ]
                    [
                        \textbf{Safety  (\S \ref{sec:safety})}, fill=constraint
                        [
                            SafeDPO~\cite{kim2025safedpo}{, }
                            SACPO~\cite{akifumi2024stepwise}{, }
                            C-DPO~\cite{liu2024enhancing}{, }
                            ADPO~\cite{kim2024adversarial}{, }
                            \citet{lee2024amechanistic}{, }
                            \citet{zhang2025backtracking}
                            , leaf, text width=64em
                        ]
                    ]
                ]
                [
                    \textbf{Model Property (\S \ref{sec:model})}, fill=model
                    [
                        \textbf{Generation  (\S \ref{sec:generation})}, fill=model
                        [
                            \textbf{Distribution}, fill=model
                            [
                                NS-DPO~\cite{son2024right}{,} 
                                SRPO~\cite{choi2025selfimproving}{,}
                                SELM~\cite{rafailov2024direct}{,}
                                e-DPO~\cite{fisch2024robust}{,}
                                \citet{lin2024limited}{,}
                                \citet{tajwar2024preference}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Length}, fill=model
                            [
                                RRHF~\cite{yuan2023rrhf}{,} 
                                R-DPO~\cite{park2024disentangling}{,} 
                                SimPO~\cite{Meng2024simpo}{,} 
                                SamPO~\cite{lu2024eliminating}{,} 
                                DMPO~\cite{shi2024direct}{,} 
                                LIFT~\cite{yuan2024following}{,} 
                                LN-DPO~\cite{ahrabian2024hitchhiker}{,} 
                                LD-DPO~\cite{liu2024length}{,} \\
                                D$^2$PO~\cite{shao2025earlier}{,} 
                                LongPO~\cite{chen2025longpo}{,} 
                                \citet{singhal2024a}{,} 
                                \citet{richardson2024declarative}
                                , leaf
                            ]
                        ]
                    ]
                    [
                        \textbf{Optimization  (\S \ref{sec:optimization})}, fill=model
                        [
                            \textbf{Likelihood}, fill=model
                            [                            
                                APO~\cite{doosterlinck2024anchored}{,}
                                DPO-Positive~\cite{pal2024smaug}
                                e-DPO~\cite{fisch2024robust}{,} 
                                Flex-DPO~\cite{yan2025dproperties}{,} 
                                \citet{rafailov2024from}{,}
                                \citet{feng2024towards}{,}
                                \citet{yuan2025common}{,} \\
                                \citet{razin2024unintentional}{,}
                                \citet{shi2024understanding}
                                , leaf
                            ]
                        ]
                        [
                            \textbf{Alignment}, fill=model
                            [
                                PAFT~\cite{pentyala2024paft}{,} 
                                \citet{lin2024mitigating}{,} 
                                \citet{thakkar2024deep}{,} 
                                \citet{lu2024online}{,}
                                \citet{chen2024preference} 
                                , leaf
                            ]
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{A taxonomy of DPO. We categorize existing DPO works into four branches: \textit{data strategy}, \textit{learning framework}, \textit{constraint mechanism}, and \textit{model property}. Different colored boxes indicate different categories and their corresponding representative references.}
    \vspace{-0.4cm}
    \label{fig:overview}
\end{figure*}

==> taxonomy.tex <==
% First, define your custom colours
\definecolor{pre}{HTML}{f95738}  % dark red
\definecolor{RLVR}{HTML}{bdd5ea}      % light blue
% \definecolor{db}{HTML}{E8F5E9}
% \definecolor{align}{HTML}{FDE2E0}
% \definecolor{tool}{HTML}{FFF9C4}
%\definecolor{tool}{HTML}{FFF9C4}
\definecolor{hidden-red}{RGB}{205, 44, 36}
\definecolor{hidden-blue}{RGB}{194,232,247}
\definecolor{hidden-orange}{RGB}{243,202,120}
\definecolor{hidden-green}{RGB}{144,238,144}
\definecolor{hidden-pink}{RGB}{255,245,247}
\definecolor{hidden-black}{RGB}{20,68,106}

\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    % line width=0.8pt,
]
\tikzstyle{leaf}=[
    my-box, 
    minimum height=1.5em,
    % fill=hidden-orange!60, 
    fill=hidden-green!50, 
    text=black,
    align=left,
    font=\normalsize,
    % font=\scriptsize,
    inner xsep=2pt,
    inner ysep=10pt,
    % line width=0.8pt,
]


% Define new styles for each branch (applied to both parent and child nodes)
\tikzstyle{train_free}=[leaf, fill=trainfreeColor!50]
\tikzstyle{train}=[leaf, fill=trainColor!50]


\begin{figure*}[t!]
    \vspace{-2mm}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                child anchor=west,
                parent anchor=east,
                grow'=east,
                anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-black,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=9em,font=\normalsize,}{},
            where level=2{text width=15em,font=\normalsize,}{},
            where level=3{text width=14em,font=\normalsize,}{},
            where level=4{text width=10em,font=\normalsize,}{},
            [
                RL enhanced LLMs, ver % common parent; keep default style
                [
                    ~Pre-training~(\S\ref{sec3.1}), pre
                    [
                        ~RL in Pre-training Loop~(\S\ref{sec3.1}), pre
                        [
                            Reinforcement Pre-Training~\citep{dong2025reinforcement}{,} 
                            OctoThinker~\citep{wang2025octothinker}{,}  
                            Visual Pre-Training~\citep{ghosh2025visual}{,} { etc.}
                            , pre, text width=45.6em 
                        ]
                    ]

                ]
                
                [
                    ~Alignment~(\S\ref{sec3}), align
                    [
                        ~Classic Algorithms~(\S\ref{sec3.2}), align
                        [
                            RLHF and Reward Modeling , align 
                            [
                                InstructGPT~\citep{ouyang2022training}{,} 
                                Bai et al.~\citep{bai2022training}{,} 
                                Text2Reward ~\citep{xie2023text2reward}{,}  
                                Xiong et al.~\citep{xiong2023iterative}{,}  
                                Eureka~\citep{ma2023eureka}{,}  
                                Kwon et al.~\citep{kwon2023reward}{,} { etc.}
                                , align, text width=45.6em 
                            ]
                            Preference Optimization , align  
                            [
                                DPO~\citep{rafailov2023direct}{,} 
                                KTO~\citep{ethayarajh2024kto}{,} 
                                $\Psi$PO~\citep{azar2024general}{,}  
                                Smaug~\citep{pal2024smaug}{,}  
                                $\beta$-DPO~\citep{NEURIPS2024_ea888178}{,}  
                                SPO~\citep{swamy2024minimaximalist}{,}  
                                ORPO~\citep{hong2024orpo}{,} { etc.}
                                , align, text width=45.6em 
                            ]
                            AI Feedback: Constitutional AI/RLAIF , align 
                            [
                                Constitutional AI~\citep{bai2022constitutional}{,} 
                                RLAIF~\citep{lee2023rlaif}{,} { etc.}
                                , align, text width=45.6em 
                            ]
                        ]
                        
                    ]
                    [
                        ~New Methods4RM Design~(\S\ref{sec3.3}), align
                        [
                            Principle/AI-generated Rewards , align 
                            [
                                RewardAnything~\citep{yu2025rewardanything}{,} 
                                AUTORULE~\citep{wang2025autorule}{,} 
                                Generalist Reward Models~\citep{li2025generalist}{,} { etc.}
                                , align, text width=45.6em 
                            ]
                            Reasoning Reward Model , align 
                            [
                                RRMs~\citep{guo2025reward}{,} 
                                GenPRM~\citep{zhao2025genprm}{,} 
                                RM-R1~\citep{chen2025rm}{,} 
                                Wang et al.~\citep{wang2025unified}{,} 
                                Liu et al.~\citep{liu2025inference}{,} { etc.}
                                , align, text width=45.6em 
                            ]
                        ]
                    
                    ]       
                ]

                [
                    ~RLVR~(\S\ref{sec4}), RLVR
                    [
                        ~Algorithmic Advances~(\S\ref{sec4.2}), RLVR
                        [
                            Type R1 and its improvements , RLVR 
                            [
                                GRPO~\citep{shao2024deepseekmath}{,} 
                                Deepseek R1~\citep{guo2025deepseek}{,} 
                                DAPO~\citep{yu2025dapo}{,}  
                                Hu et al.~\citep{hu2025open}{,}  
                                X-Reasoner~\citep{liu2025x}{,}  
                                TANGO~\citep{zha2025rl}{,}  
                                Zhou et al.~\citep{zhou2025reinforcing}{,}  
                                Kimina-Prover~\citep{wang2025kimina}{,}  
                                Magistral~\citep{rastogi2025magistral}{,}  
                                MiniMax-M1~\citep{chen2025minimax}{,}  
                                GSPO~\citep{zheng2025group}{,} { etc.}
                                , RLVR , text width=45.6em 
                            ]
                            Hybrid learning strategy , RLVR  
                            [
                                Zhang et al.~\citep{zhang2025distill}{,} 
                                Yan et al.~\citep{yan2025learning}{,} 
                                SuperRL~\citep{liu2025superrl}{,}  
                                KDRL~\citep{xu2025kdrl}{,} { etc.}
                                , RLVR, text width=45.6em 
                            ]
                            Adversarial/Structured/Multi-agent, RLVR 
                            [
                                SPIRAL~\citep{liu2025spiral}{,} 
                                R2-Reasoner~\citep{shao2025route}{,} 
                                Graph-R1~\citep{luo2025graph}{,} { etc.}
                                , RLVR, text width=45.6em 
                            ]
                            Tree structure, RLVR 
                            [
                                ToTRL~\citep{wu2025totrl}{,} 
                                TreeRPO~\citep{yang2025treerpo}{,} 
                                TreeRL~\citep{hou2025treerl}{,} { etc.}
                                , RLVR, text width=45.6em 
                            ]
                        ]
                        ~Multimodal reasoning~(\S\ref{sec4.3}), mul
                        [
                            Vision-language reasoning , mul
                            [
                                Vision-R1~\citep{huang2025vision}{,} 
                                VLM-R1~\citep{shen2025vlm}{,} 
                                Deng et al.~\citep{deng2025boosting}{,}  
                                Ma et al.~\citep{ma2025deepperception}{,}  
                                Zhou et al.~\citep{zhou2025r1}{,}  
                                VisuLogic~\citep{xu2025visulogic}{,}  
                                R1-VL~\citep{zhang2025r1}{,}  
                                GLM-4.1V-Thinking~\citep{hong2025glm}{,} { etc.}
                                , mul, text width=45.6em 
                            ]
                           Video/Spatial and Embodied Reasoning , mul  
                            [
                                Video-R1 ~\citep{feng2025video}{,} 
                                TinyLLaVA-Video-R1~\citep{zhang2025tinyllava}{,} 
                                3D-R1~\citep{huang20253d}{,}  
                                Liao et al.~\citep{liao2025improved}{,}  
                                Ouyang et al.~\citep{ouyang2025spacer}{,}  
                                Embodied-R~\citep{zhao2025embodied}{,}  
                                Ego-R1~\citep{tian2025ego}{,}
                                VAU-R1~\citep{zhu2025vau}{,} { etc.}
                                , mul, text width=45.6em 
                            ]
                            o3 style, mul
                            [o3-o4-mini-system-card, zheng2025deepeyes, zhan2025gthinker
                                GPT o3~\citep{o3-o4-mini-system-card}{,} 
                                DeepEyes~\citep{zheng2025deepeyes}{,} 
                                GThinker~\citep{zhan2025gthinker}{,} { etc.}
                                , mul, text width=45.6em 
                            ]
                            Generation and pure vision, mul
                            [
                                T2I-R1~\citep{jiang2025t2i}{,} 
                                DanceGRPO~\citep{xue2025dancegrpo}{,} 
                                Visual Planning~\citep{xu2025visual}{,} { etc.}
                                , mul, text width=45.6em 
                            ]
                            Enhanced reasoning, mul
                            [
                                Hint-GRPO~\citep{huang2025boosting}{,} 
                                Liu et al.~\citep{liu2025more}{,} 
                                SRPO~\citep{wan2025srpo}{,} 
                                Wang et al.~\citep{wang2025vicrit}{,} 
                                VGR~\citep{wang2025vgr}{,} { etc.}
                                , mul, text width=45.6em 
                            ]
                            Tasks in professional fields, mul
                            [
                                VLN-R1~\citep{qi2025vln}{,} 
                                Chen et al.~\citep{chen2025compile}{,} 
                                VAU-R1~\citep{zhu2025vau}{,} 
                                ARMed~\citep{liu2025breakingrewardcollapseadaptive}{,} 
                                CAD-Coder~\citep{guan2025cad}{,} { etc.}
                                , mul, text width=45.6em 
                            ]
                        ]                        
                    ]
                    [
                        ~Adaptive thinking~(\S\ref{sec4.4}), at
                        [
                            Length Penalty , at
                            [
                                S1~\citep{muennighoff2025s1}{,} 
                                L1~\citep{aggarwal2025l1}{,} 
                                Shorterbetter~\citep{yi2025shorterbetter}{,} { etc.}
                                , at, text width=45.6em 
                            ]
                            Thinking Mode&Difficulty-awareness , at
                            [
                                AdaptThink~\citep{zhang2025adaptthink}{,} 
                                AdaCoT~\citep{chen2025rm}{,} 
                                Zhang et al.~\citep{zhang2025continue}{,}
                                Wang et al.~\citep{wang2025adaptive}{,} { etc.}
                                , at text width=45.6em 
                            ]
                            GRPO-Variant , at
                            [
                                Ada-GRPO~\citep{guo2025reward}{,} 
                                DeGRPO~\citep{fang2025thinkless}{,}  
                                HGPO~\citep{jiang2025think}{,} 
                                Wang et al.~\citep{wang2025unified}{,}{ etc.}
                                , at text width=45.6em 
                            ]
                        ]
                    
                    ]   
                    [
                        ~Agents/Tool-use~(\S\ref{sec4.5}), agent
                        [
                            Tool/Action Space RLVR  , agent
                            [
                                AGILE ~\citep{peiyuan2024agile}{,} 
                                ToRL~\citep{li2025torl}{,} 
                                ReTool~\citep{feng2025retool}{,}
                                OpenThinkImg~\citep{su2025openthinkimg}{,} 
                                Tool-Star~\citep{dong2025tool}{,} { etc.}
                                , agent, text width=45.6em 
                            ]
                            Long-term Reward Design , agent
                            [
                                LARM~\citep{li2024larm}{,} 
                                RAGEN~\citep{wang2025ragen}{,} 
                                ShopR1~\citep{zhang2025shopr1rewardingllmssimulate}{,}
                                Zhang et al.~\citep{zhang2025divide}{,}
                                SPA-RL~\citep{wang2025spa}{,}
                                Feng et al.~\citep{feng2025group}{,} { etc.}
                                , agent text width=45.6em 
                            ]
                        ]
                    [
                        ~RLIF/Internal Feedback~(\S\ref{sec4.5}), RLIF
                        [
                            Internal Signal Reward , RLIF
                            [
                                Kang et al.~\citep{kang2025scalable}{,} 
                                Li et al.~\citep{li2025confidence}{,} 
                                van Niekerk et al.~\citep{vanniekerk2025posttraininglargelanguagemodels}{,} 
                                Zhang et al.~\citep{zhang2025no}{,} { etc.}
                                , RLIF, text width=45.6em 
                            ]
                            Self-generation Optimization , RLIF
                            [
                                TTRL~\citep{zuo2025ttrl}{,} 
                                Zhao et al.~\citep{zhao2025absolute}{,} 
                                Zhao et al.~\citep{zhao2025learning}{,}
                                SLOT~\citep{hu2025slot}{,} { etc.}
                                , RLIF text width=45.6em 
                            ]
                        ]
                    ]
                    [
                        ~Experimental Findings~(\S\ref{sec4.1}), ef
                        [
                            Sampling & Capability Boundaries , ef
                            [
                                Yue et al.~\citep{yue2025does}{,} 
                                ProRL~\citep{liu2025prorl}{,} 
                                Liu et al.~\citep{liu2025there}{,} 
                                Zhao et al.~\citep{zhao2025echo}{,} 
                                Shah et al.~\citep{shah2025rethinking}{,} 
                                Wu et al.~\citep{wu2025invisible}{,}{ etc.}
                                , ef, text width=45.6em
                            ]
                            Training Dynamics & Entropy Signals , ef
                            [
                                Cui et al.~\citep{cui2025entropy}{,} 
                                Li et al.~\citep{li2025think}{,} 
                                Ma et al.~\citep{ma2025reasoning}{,} 
                                Samineni et al.~\citep{samineni2025rl}{,} 
                                Bogdan et al.~\citep{bogdan2025thought}{,} 
                                He et al.~\citep{he2025response}{,} 
                                Chen et al.~\citep{chen2025sft}{,} 
                                Wang et al.~\citep{wang2025beyond}{ etc.}
                                , ef, text width=45.6em
                            ]
                            Data & Reward Conditions , ef
                            [
                                Wu et al.~\citep{wu2025reasoning}{,} 
                                Zhu et al.~\citep{zhu2025surprising}{,} 
                                Shojaee et al.~\citep{shojaee2025illusion}{,} { etc.}
                                , ef, text width=45.6em
                            ]
                        ]
                    ]
                [
                    ~Datasets \& Benchmarks~(\S\ref{sec5}), db
                    [
                        Synthetic Data Generation , db
                        [
                            Zhu et al.~\citep{askell2021general}{,} 
                            Goldie et al.~\citep{goldie2025synthetic}{,} 
                            Synthetic Data RL~\citep{guo2025synthetic}{,} 
                            SwS~\citep{liang2025sws}{,} { etc.}
                            , db, text width=45.6em
                        ]
                        Alignment/Dialogue , db
                        [
                            HHH~\citep{askell2021general}{,} 
                            HH-RLHF~\citep{bai2022training}{,} { etc.}
                            , db, text width=45.6em
                        ]
                        Code , db
                        [
                            APPS~\citep{dou2024stepcoder}{,} 
                            Livecodebench~\citep{jain2024livecodebench}{,} 
                            SWE-bench~\citep{lewkowycz2022solving}{,} 
                            SWE-bench Verified~\citep{yang2025swe}{,} 
                            OJBench~\citep{wang2025ojbench}{,} { etc.}
                            , db, text width=45.6em
                        ]
                        Math , db
                        [
                            GSM8K~\citep{cobbe2021training}{,} 
                            MATH~\citep{hendrycks2021measuring}{,} 
                            OlympiadBench~\citep{he2024olympiadbench}{,} 
                            Minerva Math~\citep{lewkowycz2022solving}{,} 
                            PolyMath~\citep{wang2025polymath}{,} 
                            AMC2023, AIME2024/2025, CNMO2024, HMMT2025 { etc.}
                            , db, text width=45.6em
                        ]
                        General Exams / Knowledge \& STEM , db
                        [
                            MMLU~\citep{hendrycks2020measuring}{,} 
                            MMLU-Pro~\citep{wang2024mmlu}{,} 
                            GPQA~\citep{rein2024gpqa}{,} 
                            SuperGPQA~\citep{du2025supergpqa}{,} 
                            TheoremQA~\citep{chen2023theoremqa}{,} 
                            Guru~\citep{cheng2025revisiting}{,} 
                            SimpleQA~\citep{wei2024measuring}{,} 
                            HLE~\citep{phan2025humanity}{,} 
                            LiveBench~\citep{White2025LiveBench}{,} 
                            PhyX~\citep{shen2025phyx}{,} 
                            BBH~\citep{srivastava2023beyond}{,} 
                            BBEH~\citep{kazemi2025big}{,} 
                            MMReason~\citep{yao2025mmreason}{,} { etc.}
                            , db, text width=45.6em
                        ]
                        Logic Reasoning , db
                        [
                            AutoLogi~\citep{zhu2025autologi}{,} 
                            ZebraLogic~\citep{lin2025zebralogic}{,} { etc.}
                            , db, text width=45.6em
                        ]
                        Tools / Multi-turn / Agent , db
                        [
                            $\tau^2$-Bench~\citep{barres2025tau}{,} 
                            ACEBench~\citep{chen2025acebench}{,} 
                            MultiChallenge~\citep{sirdeshmukh2025multichallenge}{,} { etc.}
                            , db, text width=45.6em
                        ]
                    ]
                ]
                [
                    ~Open-source Tools and Frameworks~(\S\ref{sec6}), tool
                    [
                        General\&End-to-End Frameworks , tool
                        [
                            VeRL~\citep{sheng2025hybridflow}{,}                        
                            ColossalChat~\citep{you2023colossalchat}{,}
                            DeepSpeed-Chat~\citep{yao2023deepspeed}{,}
                            TRL~\citep{vonwerra2022trl}{,}
                            RL4LMs~\citep{ramamurthy2022reinforcement}{,}
                            LlamaRL~\citep{wu2025llamarl}{,}
                            trlX~\citep{havrilla2023trlx}{,}
                            AReaL~\citep{fu2025areal}{,}
                            DistFlow~\citep{wang2025distflow}
                            OpenRLHF~\citep{hu2024openrlhf}{,}{ etc.}
                            , tool, text width=45.6em
                        ]
                        RL Training Library/Package , tool
                        [
                            Nemo RL~\citep{nemo-rl}{,}
                            FlashRL~\citep{liu2025flashrl}{,}
                            ROLL~\citep{wang2025reinforcement}{,} 
                            Yao et al.~\citep{yao2025offpolicy}{,}{ etc.}
                            , tool, text width=45.6em
                        ]
                    ]
                ]

                

            ]
        \end{forest}
    }
    %\vspace{-4mm}
    \caption{Taxonomy of RL Enhanced LLMs.}
    \label{fig:taxonomy}
    % \vspace{-3mm}
\end{figure*}
